Coupling Microscopic Mobility and Mobile Network Emulation for Pedestrian Communication Applications

Network emulation is a well-established method for demonstrating and testing real devices and mobile apps in a controlled scenario. This paper reports preliminary results for an open-source extension of the CrowNet pedestrian communication framework. It enables the interaction between simulated and real devices using the emulation feature of OMNeT++. The interaction is handled by several OMNeT++ modules that can be combined to match different use-cases. Initial timing measurements have been conducted for an example application which creates decentralized pedestrian density maps based on pedestrian communication. The results indicate that the approach is feasible for scenarios with a limited number of pedestrians. This limitation is mainly due to the real-time simulation requirements in coupled emulation.

==> tikz/dens_strat01.tex <==
\begin{tikzpicture}
  \foreach \x in {0,0.5,1,1.5,2}
  \foreach \y in {0,0.5,1,1.5,2}
  \draw[draw=black] (\x,\y) rectangle ++(0.5, 0.5);
  
  \draw[fill=orange, draw=none] (0.8,1.3) circle (0.05);
  \draw[draw=orange] (0.8,1.3) circle (0.5);
\end{tikzpicture}

==> tikz/dens_strat02.tex <==
\begin{tikzpicture}
  \foreach \x in {0,0.5,1,1.5,2}
  \foreach \y in {0,0.5,1,1.5,2}
  \draw[draw=black] (\x,\y) rectangle ++(0.5, 0.5);
  
  \draw[fill=green!100] (0.5, 1) rectangle ++(0.5,0.5);
\end{tikzpicture}

==> tikz/dens_strat03.tex <==
\begin{tikzpicture}
  \foreach \x in {0,0.5,1,1.5,2}
  \foreach \y in {0,0.5,1,1.5,2}
  \draw[draw=black] (\x,\y) rectangle ++(0.5, 0.5);
  
  \draw[fill=green!80] (0.5, 1) rectangle ++(0.5,0.5);

  \draw[fill=green!40] (0, 1) rectangle ++(0.5,0.5);
  \draw[fill=green!40] (0.5, 0.5) rectangle ++(0.5,0.5);
  \draw[fill=green!40] (0.5, 1.5) rectangle ++(0.5,0.5);
  \draw[fill=green!40] (1, 1) rectangle ++(0.5,0.5);

  \draw[fill=green!20] (0, 0.5) rectangle ++(0.5,0.5);
  \draw[fill=green!20] (0, 1.5) rectangle ++(0.5,0.5);
  \draw[fill=green!20] (1, 1.5) rectangle ++(0.5,0.5);
  \draw[fill=green!20] (1, 0.5) rectangle ++(0.5,0.5);
\end{tikzpicture}
